Self-stratifying turbidity currents

Turbidity currents, seafloor flows driven by the excess density of suspended particles, are key conveyors of sediment, nutrient, and pollutant from the continental margins to deep ocean, and pose critical submarine geohazard risks. Due to their vast scale and extreme aspect ratio, extant models are constrained to highly simplified depth-averaged theory and fail to capture observed behaviour. We propose a novel depth-averaged model capturing the internal energy balance and the vertical profiles of velocity, depth, and turbulent kinetic energy. The vertical profiles change as the current evolves: it self stratifies. This enables the critical new insight that turbidity current propagation is enabled by bidirectional cascades between mean-flow kinetic, turbulent, and gravitational potential energies. The model is generalised for fully confined `canyon' flow (no lateral overspill), and partially confined `channel' flow (lateral overspill over bounding levees). `Quasi-equilibrium' solutions for self-stratifying turbidity currents are constructed. These solutions are weekly unstable and connected to a slowly evolving manifold, wherein environmental currents are likely found. Equilibrium solutions, found for channel flow, are not stable either. Levee overspill removes dilute, low momentum fluid, rejuvenating the flow, which can cause a positive feedback loop where the fluid becomes increasingly concentrated. We test the new theory by modelling flow in the Congo canyon-channel system, for the first time simulating a supercritical turbidity current that travels 100s km to the distal reaches of a real-world system. It is shown that self-stratification enhances material and momentum fluxes, determining the environmental impacts and risks from such flows.

==> Sections/Appendicies/SteadyState.tex <==
\section{Steady Flow}

In this section we report the steady versions of \cref{eqn:1Dsys_vol_DE,eqn:1Dsys_part_DE,eqn:1Dsys_mom_DE,eqn:1Dsys_egy_DE} rearranged as evolution equations for $h$, $\Fro$, $\beta$, and $\gamma$. The denominator of the system is
\begin{multline} \label{eqn:system_denominator}
	\mathcal{D} 
	\eqdef 16 w_s^3 \sigma_{uu}^2 \sigma_{z\phi} \sigma_{u\phi} h \gamma^3 
	\Bigg(
		\sigma_{uu} \sigma_{z\phi} \ppar*{ 2 \sigma_{uk} - \beta \sigma_{uk}'} \Fro^2 \ppar*{ \Fro^2 - 1 }
	\\
		+ \beta \gamma^2 \Bigg[
			\sigma_{z\phi} \sigma_{uuu} \ppar*{2 \frac{\sigma_{uu}'}{\sigma_{uu}} - \frac{\sigma_{uuu}'}{\sigma_{uuu}}} \Fro^4 
		%\\
			+ \sigma_{z\phi} \sigma_{uuu} \ppar*{- \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} + \frac{\sigma_{uuu}'}{\sigma_{uuu}} + \frac{\sigma_{z\phi}'}{\sigma_{z\phi}}} \Fro^2
		\\
			+ \sigma_{uu} \varsigma_{zu\phi} \ppar*{+ 2 \frac{ \sigma_{u\phi}' }{ \sigma_{u\phi} } -2 \frac{ \sigma_{uu}' }{ \sigma_{uu} } -2 \frac{ \varsigma_{zu\phi}' }{ \varsigma_{zu\phi} } } \Fro^2
		%\\
			+ \varsigma_{zu\phi} \sigma_{uu} \ppar*{ - \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} + 2 \frac{\varsigma_{zu\phi}'}{\varsigma_{zu\phi}} - \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} }
		\Bigg]
	\Bigg)
\end{multline}
where primes represent differentiation with respect to $\beta$. For similarity flow 
\begin{align}\label{eqn:system_denominator_similarity}
	\mathcal{D} 
	= 32 w_s^3 \sigma_{uu}^3 \sigma_{z\phi}^2 \sigma_{u\phi} \sigma_{uk} h \gamma^3 \Fro^2 \ppar*{ \Fro^2 - 1 }
\end{align}
and consequently the system becomes singular when $\Fro \in \{-1,0,1\}$. The governing equations are
\begin{multline}
	\mathcal{D} \dv{h}{x}
	= 4 D \sqrt{2} \sigma_{uu}^{\frac{5}{2}} \beta  \gamma^{2} h w_s^{2} \sigma_{z\phi} 
	\Bigg(
		2 \sigma_{uk} \sigma_{u\phi} \sigma_{uu} \sigma_{z\phi} \Fro^2 \pbrk*{ 4 \Fro^2 - 1 }
	\\
		+ 2 \Fro^{4} \beta \gamma^{2} \sigma_{u\phi} \sigma_{uuu} \sigma_{z\phi} \pbrk*{ 3 \frac{\sigma_{uu}'}{\sigma_{uu}} - 2 \frac{\sigma_{uuu}'}{\sigma_{uuu}} }
	%\\
		+ 2 \Fro^{4} \beta \sigma_{uk} \sigma_{u\phi} \sigma_{uu} \sigma_{z\phi} \pbrk*{ \frac{\sigma_{uu}'}{\sigma_{uu}} - 2 \frac{\sigma_{uk}'} {\sigma_{uk}} }
	\\
		+ \Fro^{2} \beta  \gamma^{2} \sigma_{u\phi} \sigma_{uuu} \sigma_{z\phi} \pbrk*{ -3 \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} + \frac{\sigma_{uuu}'}{\sigma_{uuu}} + 3 \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} }
	\\
		+ \Fro^{2} \beta \sigma_{uk} \sigma_{u\phi} \sigma_{uu} \sigma_{z\phi} \pbrk*{ \frac{\sigma_{uk}'}{\sigma_{uk}} - \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} + \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} }
	\\
		+ 2 \beta  \gamma^{2} \sigma_{u\phi} \sigma_{uu} \varsigma_{zu\phi} \pbrk*{ \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} - \frac{\varsigma_{zu\phi}'}{\varsigma_{zu\phi}} } \pbrk{4 \Fro^2 - 1}
	\Bigg) S_h
\\
	+ 2 D^{3} \Fro^{2} \sqrt{2} \sigma_{uu}^{\frac{5}{2}} R \beta^{3} g h^{2} \sigma_{z\phi} \Bigg(
		2 \sigma_{uk} \sigma_{uu} \sigma_{z\phi}^{2} \Fro^{2}
	\\
		+ \pbrk*{4 \sigma_{uu}' \varsigma_{zu\phi} \sigma_{z\phi} \gamma^{2} - \sigma_{uuu}' \sigma_{z\phi}^{2} \gamma^{2} - \sigma_{uk}' \sigma_{uu} \sigma_{z\phi}^{2} } \beta \Fro^{2}
	\\
		+ 2 \beta  \gamma^{2} \sigma_{z\phi} \sigma_{uu} \varsigma_{zu\phi} \pbrk*{ \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} - \frac{\varsigma_{zu\phi}'}{\varsigma_{zu\phi}} }
	\Bigg) S_\Phi
\\
	+ 8 \sigma_{z\phi} D^{2} \beta^{2} h \gamma \Fro^{2} w_s \sigma_{uu}^{2} \Bigg(
		-2 \sigma_{uk} \sigma_{u\phi} \sigma_{uu} \sigma_{z\phi} \Fro^{2}
	\\
		+ \sigma_{u\phi} \sigma_{z\phi} \pbrk*{ \sigma_{uuu}' \gamma^{2} + \sigma_{uk}' \sigma_{uu} } \beta \Fro^{2}
	%\\
		+ 2 \varsigma_{zu\phi} \sigma_{u\phi} \sigma_{uu} \pbrk*{ \frac{\varsigma_{zu\phi}'}{\varsigma_{zu\phi}} - \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} } \beta  \gamma^{2}
	\Bigg) S_U
\\
	- 4 D^{3} \Fro^{2} \sqrt{2} \sigma_{uu}^{\frac{7}{2}} \beta^{4} \gamma^{2} h \sigma_{z\phi} \sigma_{u\phi} \Bigg( 2 \Fro^{2} \frac{\sigma_{uu}'}{\sigma_{uu}} - \frac{\sigma_{u\phi}'}{\sigma_{u\phi}} + \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} \Bigg) S_T
\end{multline}

\note{is it worth typesetting the other 3 equations? They're all this bad...}

==> Sections/BackMatterJFM.tex <==
%\backsection[Acknowledgements]{}

\backsection[Funding]{This work was supported by the Turbidites Research Group, University of Leeds (funded by AkerBP, CNOOC, ConocoPhillips, Harbour Energy, Murphy Oil, OMV, Oxy, and PetroChina); and the UK Natural Environment Research Council (R.M.D., grant number NE/S014535/1).}

\backsection[Declaration of interests]{The authors report no conflict of interest.}

\backsection[Author ORCID]{E.W.G. Skevington, \url{https://orcid.org/0000-0002-7709-9673}; R.M. Dorrell, \url{https://orcid.org/0000-0003-4257-7273}}

==> Sections/ConstantShape.tex <==
\section{Structure in similarity form}

We begin by discussing results for flows where the vertical and lateral structure is in similarity form, that is to say the values of $\xi_u$, $\xi_\phi$, and $\xi_k$ are functions of $\mathscr{y}$ and $\mathscr{z}$ alone. This constitutes a considerable simplification to the system of equations, as many of the shape factors do not vary with $x$ and $t$, and permits manipulation of the system of equations to yield useful expressions for the flow that are compact enough to be presented. We begin with a discussion of the energy transfer between the different fields, and then \note{continue}

==> Sections/Ellipticity.tex <==
\section{Properties of the time dependent system} \label{sec:time}

\subsection{Hyperbolicity, elliptic degeneracy, and singularities} \label{sec:time_elliptic}

For the remainder of this paper, we will employ the same parameter values, particle dimensions, and shape factors as developed in \cref{sec:vert}. The majority of our discussion will focus on steady state systems, however for this section we will briefly consider the properties of the time dependent system. The structure of the system \cref{eqn:1Dsys_vol,eqn:1Dsys_part,eqn:1Dsys_mom,eqn:1Dsys_egy} is that of a conservation law, and it may be manipulated and rewritten in the form 
\begin{align} \label{eqn:balancelaw_matrixform}
	\pdv{Q}{t} + A_F \pdv{Q}{x} &= A_S S,
&&\text{where}&
	Q &= \pgrp*{\begin{array}{c} h \\ \Phi \\ U \\ K \end{array}},
&
	S &= \pgrp*{\begin{array}{c} S_h \\ S_\Phi \\ S_U \\ S_T \end{array}},
\end{align}
and $A_F$ and $A_S$ are both $4 \times 4$ real valued matrices. The eigenvalues of $A_F$ determine the behaviour of the system of equations, and we briefly discuss this for an arbitrary system of the form \cref{eqn:balancelaw_matrixform}. Provided all eigenvalues $\lambda$ are real then the system is of hyperbolic type, and an initial value problem is well-posed. In this case, information is transported along characteristic trajectories with speed $\dv*{x}{t} = \lambda$. Conversely, if all of the eigenvalues are complex then the system is elliptic and the initial value problem is ill posed, instead `boundary conditions' must be imposed at both early and late times (for a problem on $(x,t) \in \Omega$ bounded, require boundary conditions along all of $\partial \Omega$). Problems of mixed-type have both real and complex eigenvalues, and require boundary conditions of appropriate type for each characteristic field. For non-linear systems ($A_F$ a function of $Q$) we may encounter systems that change type (because $\lambda$ are functions of $Q$). 

For the non-linear system we consider, similarity flow (constant shape factors) results in a hyperbolic system. Indeed, the characteristic polynomial of $A_f$ is
\begin{subequations} \label{eqn:flux_char_poly}
\begin{gather}
	P_{F4}(\lambda) = ( \lambda - \sigma_{uk} U ) \cdot P_{F3}(\lambda)
\end{gather}
where
\begin{multline}
	P_{F3}(\lambda) =
	\lambda^3
	- \pbrk*{ 2\sigma_{uu} + \sigma_{u\phi} } U \lambda^2
	+ \pbrk*{ 2\sigma_{u\phi} + 1 } \sigma_{uu} U^2 \lambda
%\\
	- \textfrac{1}{2} \pbrk*{ \sigma_{u\phi} + 1 } G^2 \lambda
	- \sigma_{u\phi}\sigma_{uu} U^3
	+ \sigma_{u\phi} U G^2
\end{multline}
is the characteristic polynomial for the three equations system \cref{eqn:1Dsys_vol,eqn:1Dsys_part,eqn:1Dsys_mom}, and
\begin{equation}
	G = \sqrt{ \sigma_{z\phi} R g h \Phi \cos\theta }.
\end{equation}
\end{subequations}
This structure arises due to the fluxes in the three equation system being independent of $K$, and we can immediately identify one eigenvalue $\lambda_K = \sigma_{uk} U$ associated with the transport of TKE, or energy more broadly. For the other eigenvalues, the exact expressions are unwieldy. Instead bounds can be established by looking for changes in sign of $P_{F3}$. Firstly,
\begin{subequations}
\begin{align}
	P_{F3}(U) &= \textfrac{1}{2} (\sigma_{u\phi} - 1) U (2 [\sigma_{uu}-1] U^2 + G^2),
\\
	P_{F3}(\sigma_{u\phi} U) &= - \textfrac{1}{2} \sigma_{u\phi}(\sigma_{u\phi} - 1) U G^2,
\end{align}
\end{subequations}
thus $\lambda_{\Phi}$ is between $U$ and $\sigma_{u\phi} U$ (using that $\sigma_{uu} \geq 1$ and $R\cos\theta \geq 0$). We identify this characteristic with the concentration field, $\Phi$, because for $\sigma_{u\phi}=1$ the corresponding characteristic equation is precisely the advection of concentration at speed $U$. For $\sigma_{u\phi} \neq 1$, the characteristic travels at a speed between that of the particles, $\sigma_{u\phi} U$, and the fluid, $U$. 
To identify the final two roots we use that, for $\sigma_{u\phi}<1$, $P_{F3}(\sigma_{u\phi} U)>0$ and $P_{F3}(U)<0$, thus by the asymptotic behaviour of $P_{F3}$ as $\lambda \to \pm \infty$ we have one root on $\lambda_- < \sigma_{u\phi} U$ and the other on $\lambda_+ > U$. Conversely, if $\sigma_{u\phi}>1$ then $P_{F3}(U)>0$ and $P_{F3}(\sigma_{u\phi} U)<0$, thus $\lambda_- < U$ and $\lambda_+ > \sigma_{u\phi} U$. In the special case of $\sigma_{u\phi}=1$ we can eliminate one root ($\lambda_\Phi = U$) and solve the quadratic as
\begin{align}
	\lambda_{\pm} = \sigma_{uu} U \pm \sqrt{ \sigma_{uu} (\sigma_{uu}-1) U^2 + G^2 }.
\end{align}
We identify $\lambda_{\pm}$ as waves of fluid volume and momentum, and when $\sigma_{uu}=1$ the speeds simplify to $\lambda_{\pm} = U \pm G$ which are exactly the characteristic speeds of the classic shallow water equations \citep{bk_Stoker_WW}.

\begin{figure}
	\includegraphics{Phasespace_v2/Temporal.png}
	\caption{(a) The surface on which the determinant of the characteristic polynomial equals zero. (b) The surface on which the characteristic speed associated with the TKE field changes sign through infinity.}
	\label{fig:Temporal}
\end{figure}

With varying shape factors, the system becomes sufficiently complicated that an analytic investigation of the characteristics is impractical, and we resort to numerical computations of the eigenvalues of $A_F$. Due to the shape factors of \cref{sec:vert} depending on $K$, the energy equation is no longer decoupled from the other 3, and we have to investigate the full four equation system together. This presents a potential issue. The speeds $\lambda_K$ and $\lambda_\Phi$ from the constant shape factor case take very similar values, and this makes them vulnerable to becoming a repeated root, and then it only takes a very minor alteration to $P_{F4}$ for the real roots to become a pair of complex conjugate roots. Indeed, we find that there are regions of phase space where this happens. In \cref{fig:Temporal}(a) we plot the surface on which the determinant of the characteristic polynomial is zero, that is to say there is a repeated root. The system is hyperbolic across the majority of $0<\Fro<3$, $\gamma < 1$, and the surface divides the hyperbolic regime from the mixed regime. The structure of the mixed regime is complicated. There is a large portion in $\beta<10$, $\Fro>2$, which is connected by a narrow strip down to $\Fro<1$, with more fragmented pieces in the region $\beta>2$, $0.3<\gamma<2$. 

\Cref{fig:Temporal}(b) plots the surface 
\begin{align} \label{eqn:temporal_singular_TKE}
	\Fro^2 = \frac**{ \frac{\sigma_{z\phi}'}{\sigma_{z\phi}} }{\ppar*{ \frac{2}{\beta \gamma^2} - \frac{\sigma_{uu}'}{\sigma_{uu}} }}
\end{align}
on which the evolution equation for TKE becomes singular. That is to say, all the entries in the bottom row of $A_F$ diverge, which causes $\lambda_K$ to flip between $-\infty$ and $\infty$. Local to this surface, and beyond the surface (that is, $\Fro$ larger than the right hand side of \cref{eqn:temporal_singular_TKE}), the system is hyperbolic, however it is not clear that the region where the characteristic velocity is divergent or reversed is physically meaningful.

The above discussion indicates that there are significant challenges with including varying shape factors in the model. These problems are important to address, because real currents do adjust their vertical structure. They arose due to the shape factors depending on $K$, but this \emph{must} be the case because it is the turbulent diffusion which supports the particles against settling (\cref{sec:vert}). We restrict ourselves to the region $\gamma \lesssim 1$ and $\Fro \lesssim 3$, across the majority of which the system is hyperbolic.



\subsection{Properties of the front} \label{sec:time_front}

An important aspect of turbidity currents is the front, which leads the current displacing. Here a head forms, displacing the ambient sea water. This is classically included in the depth averaged formulation as a boundary condition at some point $x=x_f$, the justification of reducing this region down to a single point being that its length is of the same order as its depth, and therefore small in comparison to the overall length of the current. The classic boundary condition at this point is the Froude number condition, for example see \citet{bk_Ungarish_GCIv2}, along with \citet{ar_Benjamin_1968,ar_Huppert_1980,ar_Ungarish_2018}. Historically, models have been derived under the assumption of top-hat flow in the body of the current (\ie the portion captured by the depth- or channel-averaged equations), and specifies $\Fro$ as a function of $R$. Here we investigate the suitability of such a condition. 

We consider a current flowing over the region $0<x<x_f(t)$, and use the equations \cref{eqn:1Dsys_vol_DE,eqn:1Dsys_part_DE} to investigate the overall change in the volume and particle load, which are
\begin{subequations}
\begin{align}
	\dv{}{t} \int_0^{x_f} h \Upsilon \dd{x} 
	&= \int_0^{x_f} \ppar*{ \Upsilon S_h + h U \dv{\Upsilon}{x} } \dd{x} 
	+ \eval*{h \Upsilon U}_{x=0} 
	+ F_h,
\\
	\dv{}{t} \int_0^{x_f} h \Upsilon \Phi \dd{x} 
	&= \int_0^{x_f} \ppar*{ \Upsilon S_\Phi + \sigma_{u\phi} h U \Phi \dv{\Upsilon}{x} } \dd{x} 
	+ \eval*{\sigma_{u\phi} h \Upsilon U \Phi}_{x=0} 
	+ F_\Phi,
\end{align}
where
\begin{align}
	F_h &\eqdef \eval*{ h \Upsilon \ppar*{ \dot{x}_f - U } }_{x=x_f},
&\text{and}&&
	F_\Phi &\eqdef \eval*{ h \Upsilon \Phi \ppar*{ \dot{x}_f - \sigma_{u\phi} U } }_{x=x_f},
\end{align}
\end{subequations}
and $\dot{x}_f \eqdef \dv*{x_f}{t}$ is the speed of the front. The terms $F_h$ and $F_\Phi$ should be understood as evaluated at the interface between the body and the head, and represent the gain of fluid via turbulent mixing in the head, and the gain of sediment through intense local erosion. In the case of top-hat flow (specifically $\sigma_{u\phi}=1$), the natural conclusion is that $\dot{x}_f=U$ so that $F_h=F_\Phi=0$ and their is no gain of volume or mass through the front. However, this is known not to be the case. It has been long documented that intense mixing occurs at the front of gravity-currents in general \citep[\eg][]{bk_Simpson_GCEL}, and we should expect this to be the case in turbidity-currents also. Thus $F_h>0$ and $\dot{x}_f>U$, but this means that for non-eroding currents $\Phi=0$ at $x=x_f$, and a region of zero-concentration fluid is established in and behind the front. Such behaviour has never been observed and is unphysical, consequently frontal mixing cannot be included in a top-hat model. Instead, it has been found necessary to include empirical factors which crudely capture the effect of mixing \citep{ar_Zemach_2017}, but this is a suboptimal approach because the effect of mixing increases over time in a manner depending on the dynamics.

Instead, we can incorporate mixing or erosion in the head by taking $\sigma_{u\phi} \neq 1$ (in this paragraph all values are evaluated at $x=x_f$). In a current that is not eroding, similar to compositional currents in the laboratory, we have $F_\Phi=0$, thus $\dot{x}_f = \sigma_{u\phi} U$ and $F_h = h \Upsilon U ( \sigma_{u\phi} - 1 )$ so that for mixing ($F_h>0$) we require $\sigma_{u\phi} > 1$. For a current that purely erosional, an idealisation of some turbidity-currents, we have $F_h=0$, thus $\dot{x}_f = U$ and $F_\Phi = h \Upsilon U \Phi ( 1-\sigma_{u\phi} )$ so that for erosion ($F_\Phi>0$) we require $\sigma_{u\phi} < 1$. Thus the vertical structure acts to control, or else is determined by, the mixing and erosional dynamics at the front. In a real current it is likely that we see both mixing and erosion ($F_h>0$ and $F_\Phi>0$) so that $\dot{x}_f > \max\pbrc{ 1 , \sigma_{u\phi} } U$, and $\sigma_{u\phi}$ has a more complicated relationship between the balance of mixing and erosion.

At this stage, we can use the method of characteristics to establish the number and type of boundary conditions that should be applied. The general case is challenging. However, for similarity flow, we know that $\lambda_-<\dot{x}_f$, so we require a boundary condition determining the relationship between volume and momentum, for which a Froude number condition is appropriate. Additionally, in all cases considered $\dot{x}_f \geq \max\pbrc{ 1 , \sigma_{u\phi} } U$ so that $\lambda_\Phi<\dot{x}_f$, and a boundary condition is required specifying the effect of mixing and erosion on concentration. If $\lambda_K < \dot{x}_f$, which is very likely, then we additionally require a boundary condition describing the turbulent processes. Thus, while a Froude number condition can be used, it cannot be used in isolation, and a suite of boundary conditions are required to adequately capture the dynamics of the front.

From here on we will focus on the steady state system $\pdv*{}{t}=0$, and employ she shallow slope assumption for our calculations ($\sin\theta \sim \tan\theta \sim \theta$, $\cos\theta \sim 1$). 

==> Sections/Front.tex <==
\subsection{Properties of the front} \label{sec:time_front}

An important aspect of turbidity currents is the front. Here a head forms, displacing the ambient sea water. This is classically included in the depth averaged formulation as a boundary condition at some point $x=x_f$, the justification of reducing this region down to a single point being that its length is of the same order as its depth, and therefore small in comparison to the overall length of the current. The classic boundary condition at this point is the Froude number condition, for example see \citet{bk_Ungarish_GCIv2}, along with \citet{ar_Benjamin_1968,ar_Huppert_1980,ar_Ungarish_2018}. Historically, models have been derived under the assumption of top-hat flow in the body of the current (\ie the portion captured by the depth- or channel-averaged equations), and specify $\Fro$ as a function of $R$. Here we investigate the suitability of such a condition. 

We consider a current flowing over the region $0<x<x_f(t)$, and use the equations \cref{eqn:1Dsys_vol_DE,eqn:1Dsys_part_DE} to investigate the overall change in the volume and particle load, which are
\begin{subequations}
\begin{align}
	\dv{}{t} \int_0^{x_f} h \Upsilon \dd{x} 
	&= \int_0^{x_f} \ppar*{ \Upsilon S_h + h U \dv{\Upsilon}{x} } \dd{x} 
	+ \eval*{h \Upsilon U}_{x=0} 
	+ F_h,
\\
	\dv{}{t} \int_0^{x_f} h \Upsilon \Phi \dd{x} 
	&= \int_0^{x_f} \ppar*{ \Upsilon S_\Phi + \sigma_{u\phi} h U \Phi \dv{\Upsilon}{x} } \dd{x} 
	+ \eval*{\sigma_{u\phi} h \Upsilon U \Phi}_{x=0} 
	+ F_\Phi,
\end{align}
where
\begin{align}
	F_h &\eqdef \eval*{ h \Upsilon \ppar*{ \dot{x}_f - U } }_{x=x_f},
&\text{and}&&
	F_\Phi &\eqdef \eval*{ h \Upsilon \Phi \ppar*{ \dot{x}_f - \sigma_{u\phi} U } }_{x=x_f},
\end{align}
\end{subequations}
and $\dot{x}_f \eqdef \dv*{x_f}{t}$ is the speed of the front. The terms $F_h$ and $F_\Phi$ should be understood as evaluated at the interface between the body and the head, and represent the gain of fluid via turbulent mixing in the head, and the gain of sediment through intense local erosion. In the case of top-hat flow (specifically $\sigma_{u\phi}=1$), the natural conclusion is that $\dot{x}_f=U$ so that $F_h=F_\Phi=0$ and their is no gain of volume or mass through the front. However, this is known not to be the case. It has been long documented that intense mixing occurs at the front of gravity-currents in general \citep[\eg][]{bk_Simpson_GCEL,ar_Sher_2015}, and we should expect this to be the case in turbidity-currents also. Thus $F_h>0$ and $\dot{x}_f>U$, but this means that for non-eroding currents $\Phi=0$ at $x=x_f$, and a region of zero-concentration fluid is established in and behind the front. Such behaviour has never been observed and is unphysical, consequently frontal mixing cannot be included in a top-hat model. Instead, it has been found necessary to include empirical factors which crudely capture the effect of mixing \citep{ar_Zemach_2017}, but this is a suboptimal approach because the effect of mixing increases over time in a manner depending on the dynamics.

Instead, we can incorporate mixing or erosion in the head by taking $\sigma_{u\phi} \neq 1$ (in this paragraph all values are evaluated at $x=x_f$). 
In a current that is not eroding, similar to compositional currents in the laboratory, we have $F_\Phi=0$, thus $\dot{x}_f = \sigma_{u\phi} U$ and $F_h = h \Upsilon U ( \sigma_{u\phi} - 1 )$ so that for mixing ($F_h>0$) we require $\sigma_{u\phi} > 1$. To obtain a current with $\sigma_{u\phi} > 1$, supposing that it is stably stratified with a well mixed higher-concentration region close to the base, this well mixed region should extend above the velocity maximum. 
For a current that purely erosional, an idealisation of some turbidity-currents, we have $F_h=0$, thus $\dot{x}_f = U$ and $F_\Phi = h \Upsilon U \Phi ( 1-\sigma_{u\phi} )$ so that for erosion ($F_\Phi>0$) we require $\sigma_{u\phi} < 1$. To obtain a current with $\sigma_{u\phi} < 1$ the well mixed region should end below the velocity maximum, which is an unlikely configuration.
In a real current it is likely that we see both mixing and erosion ($F_h>0$ and $F_\Phi>0$) so that $\dot{x}_f > \max\pbrc{ 1 , \sigma_{u\phi} } U$, and $\sigma_{u\phi} \gtrsim 1$ has a more complicated relationship between the balance of mixing and erosion. Thus the vertical structure acts to control, or else is determined by, the mixing and erosional dynamics at the front.

The link between flow speed and entrainment/erosion at the front gives insight into a difference between laboratory and environmental currents, recalling that the standard measure of velocity is the Ellison-Turner velocity $\breve{U} = \sigma_{uu} U$ (\cref{app:ETshape}). In laboratory flows typically $\dot{x}_f<\breve{U}$, while in environmental scale flows it is possible for $\dot{x}_f>\breve{U}$ as shown by \citet{ar_Zabala_2017}. This is a crucial distinction, showing that in laboratory scale flows the head is weekly entraining/eroding, while in environmental scale flows these processes can be very strong, which gives a potential reason for the substantially different flow structures in these two settings in terms of the dynamics local to the head.

At this stage, we can use the method of characteristics to establish the number and type of boundary conditions that should be applied, a boundary condition required at $x_f$ for characteristics with $\lambda < \dot{x}_f$. The general case is challenging. However, for similarity flow, we know that $\lambda_-<\dot{x}_f$, so we require a boundary condition determining the relationship between volume and momentum, for which a Froude number condition is appropriate. Additionally, in all cases considered $\dot{x}_f \geq \max\pbrc{ 1 , \sigma_{u\phi} } U$ so that $\lambda_\Phi<\dot{x}_f$, and a boundary condition is required specifying the effect of mixing and erosion on concentration. If $\lambda_K < \dot{x}_f$, which is very likely as we expect $\sigma_{uk}<1$, then we additionally require a boundary condition describing the turbulent processes. Thus, while a Froude number condition can be used, it cannot be used in isolation, and a suite of boundary conditions are required to adequately capture the dynamics of the front. 

==> Sections/FrontMatterJFM.tex <==
\title{Self-stratifying turbidity currents}
\shorttitle{Self-stratifying turbidity currents}

\author{Edward W.G. Skevington\aff{1}\corresp{\email{e.w.skevington@hull.ac.uk}} \and Robert M. Dorrell\aff{1}}
\shortauthor{E.W.G. Skevington and R.M. Dorrell}
\affiliation{
	\aff{1} Energy and Environment Institute, University of Hull, HU6 7RX, England
}

\maketitle

\begin{abstract}
	Turbidity currents, seafloor flows driven by the excess density of suspended particles, are key conveyors of sediment, nutrient, and pollutant from the continental margins to deep ocean, and pose critical submarine geohazard risks. Due to their vast scale and extreme aspect ratio, extant models are constrained to highly simplified depth-averaged theory and fail to capture observed behaviour. We propose a novel depth-averaged model capturing the internal energy balance and the vertical profiles of velocity, depth, and turbulent kinetic energy. The vertical profiles change as the current evolves: it self stratifies. This enables the critical new insight that turbidity current propagation is enabled by bidirectional cascades between mean-flow kinetic, turbulent, and gravitational potential energies. 

	The model is generalised for fully confined ‘canyon’ flow (no lateral overspill), and partially confined ‘channel’ flow (lateral overspill over bounding levees). ‘Quasi-equilibrium’ solutions for self-stratifying turbidity currents are constructed. These solutions are weekly unstable and connected to a slowly evolving manifold, wherein environmental currents are likely found. Equilibrium solutions, found for channel flow, are not stable either. Levee overspill removes dilute, low momentum fluid, rejuvenating the flow, which can cause a positive feedback loop where the fluid becomes increasingly concentrated. We test the new theory by modelling flow in the Congo canyon-channel system, for the first time simulating a supercritical turbidity current that travels 100s \unit{km} to the distal reaches of a real-world system. It is shown that self-stratification enhances material and momentum fluxes, determining the environmental impacts and risks from such flows. 
\end{abstract}

==> Sections/Overspill.tex <==
\section{Levee overspill}

==> Sections/Parameters.tex <==
\section{Parameter values}

\begin{planlist}
    \item Give parameter values for Congo system
\end{planlist}

\note{these should be integrated into the text somewhere}

\begin{align}
	d &= 10^{-5}
\\
	\nu &= 10^{-6}
\\
	\rho &= 1000
\\
	\rho_p &= 2600
\\
	g &= 9.8
\\
	\gamma_\equl &= 1
\\
	\tilde{C}_d &= 1/40^2
\\
	\Sch_\phi &= 0.1
\end{align}

The equilibrium in \cref{eqn:eddy_viscosity_coefficient} is computed at $\gamma=\gamma_{\equl}$, $\beta=0$. Simulations run in shallow limit, that is $\sin\theta \sim \tan\theta \sim \theta$, $\cos\theta \sim 1$.


\note{Discuss size of $C_d$, why small? Abad 2011 for size of $C_z$}

\note{Can we do bigger particles? If not why not?}

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
    	{\eval@wdot*{#3}}
   		{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}
\DeclarePairedDelimiter{\shock}{[}{]_{-}^{+}}




%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}




%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
	\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
	\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
	\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
	\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
	\newcommand\Ric{\mbox{\textit{Ri}}}
\fi

%\Sch Richardson number
\ifdefined\Sch\else
	\newcommand\Sch{\mbox{\textit{Sc}}}
\fi



%---VECTOR---
\newcommand*\vecb[1]{\bm{#1}}
\newcommand*\vecbu[1]{\hat{\vecb{#1}}}
\newcommand*\dotp{\mathpalette\omitdummy@{0.5}}
\newcommand*\ddotp{\bm{:}}




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%For mixed partial derivative d2f/dxdy, use \pdvt three arguments for f,x,y
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
    	{\frac@starwdot*{#3}{#4}}
    	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\mathrm{d} #3%
	}{%
		\mathrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\mathrm{d}^{#1} #2}{{\mathrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\mathrm{d}^{#2} #4}{{\mathrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\else
			\frac*[#2]{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
			\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%\pdvt
\NewDocumentCommand\pdvt@nostar{mmm}{%
	\frac@nostar{\partial^2 #1}{\partial #2 \partial #3}
}
\NewDocumentCommand{\pdvt@star}{sO{}mmm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^2 #3}{\partial #4 \partial #5}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^2 #3}{\partial #4 \partial #5}%
		\else
			\frac*[#2]{\partial^2 #3}{\partial #4 \partial #5}%
		\fi
	}%
}
\newcommand*\pdvt{\@ifstar{\pdvt@star}{\pdvt@nostar}}



%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
%	\frac{\partial^2 #2}{\partial #3 \partial #4}
%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
%	|#1,#2,#3,#4,#5|
%%	\IfBooleanTF{#2}{%
%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
%%	}{%
%%		\if \relax\detokenize{#3}\relax
%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
%%		\else
%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
%%		\fi
%%	}%
%}
%\newcommand*\pdvm@nostar[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm@STAR[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
%	F|#1,#2,#3,#4,#5|
%}
%
%\newcommand*\pdvm@nostar[1]{%
%	A|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@frac}{}%
%	\fi%
%}
%\newcommand*\pdvm@star[2]{%
%	B%\abs{ #1 , #2 } \:
%%	\ifnum #2=2
%%		\pdvm@two{\pdvm@str@slsh}{#1}%
%%	\fi%
%}
%\newcommand*\pdvm@sstar[1]{%
%	C|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@flat}{}%
%	\fi%
%}
%
%\newcommand\pdvm@staropt[1][]{%
%	a| #1 | \:%
%	\if \relax\detokenize{#1}\relax
%		b%
%		\pdvm@star{}%
%	\else
%		c%
%		\pdvm@star{#1}%
%	\fi
%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}



%---VECTOR CALCULUS---
%Uses similar syntax to the physics package.
%
%\grad{f}	Gradient operator
%\div{f}	Divergence operator
%\curl{f}	Curl operator

\let\divisionsymbol\div

\newcommand\grad[1]{\nabla #1}
\renewcommand\div[1]{\nabla \dotp #1}
\newcommand\curl[1]{\nabla \times #1}





%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
		\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
  	\mathchoice
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
    	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
    	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
  	}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%%Upright math text
%\DeclareMathAlphabet{\mathup}{OT1}{\familydefault}{m}{n}

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\@ifundefined{eqdef}{\newcommand{\eqdef}{\vcentcolon =}}{}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}

%Degree symbol
\newcommand{\degree}{^{\circ}}



%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
%No braces
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
%Left braced
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
%Left braced with display style
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
}{
	\end{array}\right.
}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
				\setlength{\sbsse@Wd}{\sbsse@We/3}
				\hspace{\sbsse@Wd}
			\else
				\setlength{\sbsse@Wd}{\sbsse@We/4}
				\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
